Probing Script Knowledge from Pre-Trained Models

Script knowledge is critical for humans to understand the broad daily tasks and routine activities in the world. Recently researchers have explored the large-scale pre-trained language models (PLMs) to perform various script related tasks, such as story generation, temporal ordering of event, future event prediction and so on. However, it's still not well studied in terms of how well the PLMs capture the script knowledge. To answer this question, we design three probing tasks: inclusive sub-event selection, starting sub-event selection and temporal ordering to investigate the capabilities of PLMs with and without fine-tuning. The three probing tasks can be further used to automatically induce a script for each main event given all the possible sub-events. Taking BERT as a case study, by analyzing its performance on script induction as well as each individual probing task, we conclude that the stereotypical temporal knowledge among the sub-events is well captured in BERT, however the inclusive or starting sub-event knowledge is barely encoded.

==> 1introduction_backup.tex <==
\section{Introduction}

Scripts~\cite{schank2013scripts} are knowledge of the stereotypical event sequences happening under a scenario.
Scripts captures humans' knowledge of procedures in a wide range of domains from daily lives to scientific processes.
For example, a classic example of scripts is the \emph{Eating in a Restaurant} script that consists of the event chain of \emph{Enter}$\rightarrow$\emph{Order}$\rightarrow$\emph{Eat}$\rightarrow$\emph{Pay (and Tip)}$\rightarrow$\emph{Leave}.

% They are related to structured sequences of
% participants and events that have been called scripts.
% These participants and events can be filled in and
% instantiated in a particular text situation to draw inferences. 

Script knowledge -- importance and applications
chains of events
the containing , temporal and causal under a theme
narrative understanding
narrative does not describe all the details but the omitted details are necessary for understanding the texts in-depth.
Like the example people use to criticize AI/NLP progresses all the time~\cite{ai30}:\mo{I will try another example with a useful script latter, maybe as a teaser figure.}

    {\small
    \centering
    \begin{tabular}{p{7.3cm}}
      \rowcolor{Gray} \textbf{{Story}:} \textit{A man went into a restaurant and ordered a hamburger, cooked rare. When it arrived, it was burned to a crisp. The waitress stopped by the man's table.“Is burger okay?” she asked.“Oh, it's just great,”the man said, pushing back his chair and storming out of the restaurant without paying. The waitress yelled after him,“Hey, what about the bill?”}\\ 
      \rowcolor{Gray} \textbf{Question:} Did the man eat the hamburger?)
      \end{tabular}\\}

Recent pre-training techniques~\cite{bert,gpt,bart} give powerful models for NLP research. Works has demonstrated that these models either directly capture certain types of important commonsense knowledge~\cite{petroni-etal-2019-language} or consists of the necessary inductive biases~\cite{huang,yejin2022aclsubmission} to make them learn to acquire such knowledge fast.
These studies covered wide commonsense knowledge types such as entity relations and event relations.
However, as another important type of commonsense knowledge, whether the script knowledge is also well captured by the pre-trained models remains unstudied. 
% -- extraction of chains from texts}

We set up the first task and benchmarks for script knowledge probing from pre-trained models.
We then investigate the research problem in two folds:

\vspace{-5pt}
\begin{itemize}[leftmargin=*]
\setlength\itemsep{0em}
\item \emph{Whether and what script knowledge exists in the pre-trained models.} To this end, we choose the key sub-tasks in script generation, \textbf{sub-event selection} (i.e., sub-event relation) and \textbf{sub-event ordering} (i.e., temporal relation). On these sub-tasks, we studied the usage of different prompting methods, from hand-written prompts to learned prompts, to query the knowledge from pre-trained language models. By investigating their performance gaps to the fine-tuning results, we find that the sub-event selection sub-task has relatively poor performance. This indicates the lack of the sub-event relation knowledge in the pre-trained models.

\item \emph{How to better generate the scripts from these pre-trained models.} The previously defined sub-tasks, i.e., sub-event selection and ordering, have been studied in different settings from ours. However, none of previous work studied the generation and evaluation of the whole scripts. Furthermore, we show that these sub-tasks, even well-solved, are not sufficient for accurately generating the whole event sequences, which is the ultimate goal of script generation. We propose an auto-regressive approach for this problem. Our approach starts with a new \textbf{starting sub-event selection} sub-task and the corresponding prompting method, then generate the following sub-events step-by-step. Experiments show that our approach extracts whole scripts with advanced performance.
\end{itemize}


% ===========Goal =============

% (1) Probing with Prompts: whether the pre-trained language models, e.g., BERT, RoBERTa, GPT, can capture the script knowledge. Investigate the difference among all the pre-trained language models, and try different prompt templates.

% (2) Prompt tuning to better capture the script knowledge: 
